Towards pandemic preparedness: ability to estimate high-resolution social contact patterns from longitudinal surveys

Social contact surveys are an important tool to assess infection risks within populations, and the effect of non-pharmaceutical interventions on social behaviour during disease outbreaks, epidemics, and pandemics. Numerous longitudinal social contact surveys were conducted during the COVID-19 era, however data analysis is plagued by reporting fatigue, a phenomenon whereby the average number of social contacts reported declines with the number of repeat participations and as participants' engagement decreases over time. Using data from the German COVIMOD Study between April 2020 to December 2021, we demonstrate that reporting fatigue varied considerably by sociodemographic factors and was consistently strongest among parents reporting children contacts (parental proxy reporting), students, middle-aged individuals, those in full-time employment and those self-employed. We find further that, when using data from first-time participants as gold standard, statistical models incorporating a simple logistic function to control for reporting fatigue were associated with substantially improved estimation accuracy relative to models with no reporting fatigue adjustments, and that no cap on the number of repeat participations was required. These results indicate that existing longitudinal contact survey data can be meaningfully interpreted under an easy-to-implement statistical approach adressing reporting fatigue confounding, and that longitudinal designs including repeat participants are a viable option for future social contact survey designs.

==> safekeeping.tex <==
\subsection*{The Bayesian Rate Consistency model for estimating social contacts}

Here, we provide a concise introduction of the Bayesian Rate Consistency (BRC) model\cite{dan_estimating_2023}. Our objective is to estimate the contact intensity (the anticipated number of contacts on a per-individual basis) between genders, represented by superscripts $g,h \in \{M,F\}$, across one-year age brackets, represented by subscripts $a,b \in B=\{0,1,2,\ldots,84\}$, during survey wave $t=1,2,\ldots$. It is important to underline that the set $B$ is limited to ages 0 through 84. This choice arises from the age aggregation strategy and the age-specific sample size of COVIMOD; however, it is adaptable for analysis in different studies.

The variable $Y_{tab}^{gh}$ denote the cumulative number of contacts by participants of gender $g$ and age $a$ with individuals of gender $h$ and age $b$ during survey wave $t$. To model this count data, we employ an overdispersion adjusting Negative Binomial observation model as follows:
\begin{subequations}\label{lkl-contact-patterns}
\begin{align}
Y_{tab}^{gh} & \sim \text{NegBinomial}\left(\alpha_{tab}^{gh}, \frac{\odisp}{1+\odisp}\right),\\
\mu_{tab}^{gh} & = \alpha_{tab}^{gh}\odisp,\\
\log \mu_{tab}^{gh} & = \log m_{tab}^{gh} + \log \Part + \log S_{ta}^g. \label{lkl-contact-patterns-b}
\end{align}
\end{subequations}
Within this context, $N_a^g$ represents the number of participants of gender $g$ and age $a$. $S_{ta}^g$ denotes the proportion of contacts reported without gender and/or age information. Here, $\mu_{tab}^{gh}$ can be interpreted as the expected number of total contacts among the respective age-gender pairs. Expressed differently, $\mu_{tab}^{gh}$ is the product of the contact intensity $m_{tab}^{gh}$ and the total participant count. We proceed to model the logarithm of the contact intensity $m_{tab}^{gh}$ using the linear function
\begin{equation}
    \log m_{tab}^{gh}= \beta_0 + \tau_t + \bmf^{gh}_t(a,b) + \log P_b^g. \label{linear-predictior}
\end{equation}
Here, $\beta_0 \in \mathbb{R}$ acts as a global baseline parameter. The parameter $\tau_t \in \mathbb{R}$ serves as an independent age-gender homogeneous survey wave effect. Given gender pairs $gh$ and survey wave $t$, $\bmf^{gh}_t(a,b)$ are 2-dimensional continuous random functions of participant age and contact age. Finally, $P_b^g$ represents the population count of people of gender $g$ and age $b$. The functions $\bmf^{gh}_t(a,b)$ were modeled using approximate zero-mean Gaussian processes (GPs). For an exact description regarding the construction of these functions, we direct readers to Dan et al.\cite{dan_estimating_2023}, Riutort-Mayol et al.\cite{riutort-mayol_practical_2022}, and Solin and Särkkä\cite{solin_hilbert_2020}.

Now, let subscript $r=0,1,2,\ldots$ denote the number of times a participant responded to the survey. To account for the effect of reporting fatigue on contact intensity, an age-gender homogeneous term $\rho_r \in \mathbb{R}, \rho_0 = 0$ is introduced such that
\begin{equation}
    \log \mu_{trab}^{gh} = \log m_{tab}^{gh} + \rho_r + \log N_{tra}^{gh}.
\end{equation}
This term captures any changes in contact intensities resulting from repeated survey participation. Consequently, this adjustment ensures that the estimated contact intensities $\log m_{tab}^{gh}$ in subsequent survey rounds are elevated, compensating for the reduced intensity implied by the original data.


In the COVIMOD study, as well as numerous other social contact studies conducted during the COVID-19 era, participants were asked to report their contacts in broad age groups defined as, 
\begin{equation}
    \begin{split}
        c\in C = \{& \text{0-4, 5-9, 10-14, 15-19, 20-24, 25-34, 35-44, 45-54, 55-64, 65-69, 70-74, 75-79, 80-84} \}.
    \end{split}
\end{equation}
Given this age grouping strategy, equation (\ref{lkl-contact-patterns}) is modified to:
\begin{equation}
    Y_{trac}^{gh} = \sum_{b \in c} Y_{trab} \sim \text{NegBinomial}\left(\sum_{b \in c} \alpha_{trab}^{gh}, \frac{\odisp}{1 + \odisp}\right).
\end{equation}\label{coarse-lkl-contact-patterns}

To fully characterize our model, standard priors were assigned to all model parameters. The model, constructed for survey waves $t=1,\dotsc,5$, reporting repeats $r=0,\dotsc,4$, genders $g,h \in {M,F}$, participant age groups $a\in A$, and population age groups $b\in B$, is presented as:

\begin{subequations} \label{eq:full-model}
\begin{align}
Y_{trac}^{gh} & \sim \text{NegBinomial}\left(\sum_{b \in c} \alpha_{trab}^{gh}, \frac{\odisp}{1+\odisp}\right)\\
\mu_{trab}^{gh}  & = \alpha_{trab}^{gh} \odisp\\
\log \mu_{trab}^{gh} & = \log m_{tab}^{gh} + \rho_r + \log \Parttr  + \log S^g_{ta}\\
\log m_{tab}^{gh} & = \beta_0 + \tau_t + \bmf_t^{gh}(a,b) + \log \Pop[b]{h} 
\end{align}
\end{subequations}
accompanied by,
\begin{subequations} \label{eq:full-model-priors}
\begin{align}
\beta_0 & \sim \text{Normal}(0, 10) \\
\rho_r & \sim \text{Normal}(0, 1) \\
\tau_t & \sim \text{Normal}(0, 1) \\
\odisp & \sim \text{Exponential}(1) \\
\bmf_{t}^{gh}(a,b)|\mgnt_{ti}, \lnsc_{ti} & \overset{\text{approx.}}\sim \text{GP}(\bm{0}, K_{\mgnt_{ti}, \lnsc_{ti}}), \quad i = 1, 2 \\
\mgnt_{ti} & \sim \text{Cauchy}^+(0,1), \quad i = 1,2  \\
\lnsc_{ti} & \sim \text{InverseGamma}(5, 5), \quad i = 1,2. 
\end{align}
\end{subequations}
It should be noted that the components of the GP covariance matrix, $K_{\mgnt_{ti}, \lnsc_{ti}}$, are computed employing the Matérn $5/2$ kernel with magnitude $\mgnt_{ti}$ and length-scale $\lnsc_{ti}$.

\subsection*{Modelling heterogeneous reporting fatigue effects}
The BRC model assumes that the effect of reporting fatigue is homogeneous irrespective of participant and contact attributes. However, this assumption is likely to be incorrect, as reporting fatigue could be influenced by factors such as age, education, and occupation\cite{kristen_backor_estimating_2007, le_when_2021}. In Table~\ref{tab:models}, we describe the three ways in which we modified the reporting fatigue term within the BRC model to reflect variations in reporting fatigue for different participant age and contact ages. While gender does influence contact counts\cite{dan_estimating_2023}, we omit the gender element from our modifications as existing literature suggests that, in the context of reporting fatigue, gender's significance pales in comparison to age and the number of repeats\cite{kristen_backor_estimating_2007, le_when_2021}.

Considering that reporting fatigue can only skew contact counts in a negative direction, we constrain $\rho_{rac}$ to the negative real axis by taking the negative of the exponent across all model variations. The term $\rho_r \in \mathbb{R}$ stands for independent baseline parameters for each survey repetition. For models A and B, $f_r(a)$ and $f_r(c')$ represent 1-dimensional continuous functions modeled using approximate zero-mean Gaussian processes\cite{dan_estimating_2023, riutort-mayol_practical_2022, solin_hilbert_2020}. However, an adaptation is required for the contact group dimension since $c \in {\text{0-4, 5-9, \ldots, 75-79, 80-84}}$ is discrete. We take the midpoint of each age group such that
\begin{equation}
    c' \in C' = \{2, 7, 12, 17, 22, 29, 39, 49, 59, 67, 72, 77, 82\}.
\end{equation}

In model C, $f_r(a,c')$ is a 2-dimensional continuous function of participant age and contact age, which is modeled in a similar fashion to those in equation \ref{linear-predictior}. This function can be interpreted as a smooth interaction term between participant age and contact age group. The covariance matrices, $K_{\alpha,l}$ and $K_{\alpha_i, l_i}$, derive from the squared-exponential kernel characterized by magnitude $\mgnt \sim \text{Cauchy}^+(0,1)$ and length-scale $\lnsc \sim \text{InverseGamma(5,5)}$, consistent with equation \ref{eq:full-model-priors}.

\begin{table}[!ht]
    \centering
    \begin{tabular}{cll}
    \toprule
        Model & Model Structure & Priors \\ \midrule
        Original & $\rho_r$ & $\rho_r \sim \text{Normal}(0,1)$ \\ \hline
        A & $\rho_{ra} = -\exp (\rho_r + f_r(a)) $ & $\rho_r \sim \text{Normal}(0,1)$ \\
          & & $f_r(a) \overset{\text{approx.}}\sim \text{GP}(0, K_{\alpha,l})$ \\ \hline
        B & $\rho_{rac} = -\exp \left( \rho_r + f_r(a) + f_r(c') \right)$ & $\rho_r \sim \text{Normal}(0,1)$  \\
          & & $f_r(a) \overset{\text{approx.}}\sim \text{GP}(0, K_{\alpha,l})$ \\
          & & $f_r(c') \overset{\text{approx.}}\sim \text{GP}(0, K_{\alpha,l})$ \\ \hline
        C & $\rho_{rac} = -\exp (\rho_r + f_r(a,c'))$ & $ \rho_r \sim \text{Normal}(0,1)$ \\
          & & $f_r(a,c') \overset{\text{approx.}}\sim\text{GP}(\bm{0}, K_{\alpha_i, l_i}), i=1,2$ \\
    \bottomrule
    \end{tabular}
    \caption{Age dependent reporting fatigue models and their prior specifications.}
    \label{tab:models}
\end{table}

\subsection*{Bayesian Inference, Model Comparison, and Model Diagnostics}


The joint posterior distribution of all parameters was sampled using the probabilistic programming language, \texttt{Stan}\cite{stan_development_team_stan_2022}, through the \texttt{cmdstanr} interface (version 0.5.2)\cite{jonah_gabry_cmdstanr_2023}. We ran eight chains concurrently, with 500 warmup iterations followed by 1000 sampling iterations. The lowest effective sample size across all three models was XYZ, and the $\hat{R}$ convergence metrics were below 1.01 for all models. This suggests that the Markov chains merged and integrated efficiently. Trace plots of the parameters with the lowest effective sample size and highest $\hat{R}$ can be found in Appendix Figure 

To assess the fit of our models to the training data, we calculate the mean-squared error (MSE) and perform posterior predictive checks (PPC). To quantitatively compare the three models outlined in Table \ref{tab:models}, we employ approximate leave-out-out expected log-posterior density (LOO-ELPD)\cite{vehtari_practical_2017}. Simply put, this is a measure of the predictive accuracy of the model to unseen data with higher scores indicating better model generalisability. Our \texttt{R} and \texttt{Stan} code, along with additional analysis scripts, can be found at \href{https://github.com/MLGlobalHealth/bayes-rate-consistency}{https://github.com/MLGlobalHealth/bayes-rate-consistency}.


We previously proposed the Bayesian Rate Consistency model (BRC)~\cite{dan_estimating_2023} to estimate contact intensity surfaces $m_{a,b}$ that quantify the average number of contacts that one individual in age group $a$ has with all individuals of age $b$, where both $a$ and $b$ are specified at fine 1-year age bands. The key point of the BRC is that in a closed population with population sizes $P_a$, the true, unobserved number of contacts is the same regardless of whether we count from $a$ to $b$ or from $b$ to $a$, i.e.
\begin{equation}\label{e:flow_identity}
    P_a m_{a,b} = P_b m_{b,a}
\end{equation}
for all $a,b$. This principle makes possible to decipher fine-age contact intensity surfaces even if the age of contacts is only reported in coarse age bands such as
\begin{equation}
c \in \mathcal{C} = \{ \text{0-4, 5-9, 10-14, 15-19, 20-24, 25-34, 35-44, 45-54, 55-64, 65-69, 70-74, 75-79, 80-84} \},
\end{equation}
by leveraging the exact age $a$ of the reporting participant. The basic BRC model was developed for aggregated contact data between age groups, $Y_{a,c}$ where $a\in\mathcal{A}=\{0,\dotsc,85\}$ and $c\in\mathcal{C}$, and therefore was unable to capture high-resolution effects corresponding to additional socio-demographic factors such as household size, employment status, or location. Here, we demonstrate that it is possible to extend the BRC to individual-level data $Y_{i,c}$ of participants $i$ at no additional computational cost, and thereby estimate high-resolution contact intensity surfaces that further account for additive socio-demographic factors. This advance is primarily due to improved indexing and bookkeeping in the code (Supplementary Text S2). The essential structure of the high-resolution BRC is
\begin{subequations}
\begin{align}
    Y_{i} &\sim \text{NegBinomial}\left( \lambda_i, \varphi \right) \quad\text{for }i=1,\ldots,N, \text{ and }  r = 1,\ldots,R \\
    \log(\lambda_i) &= \alpha + \bm{x}_i^\top \beta + f_\theta(a_i) - \rho_{j_i}(r_i),
\end{align}
\end{subequations}
where $\gamma_{i,b}$ are the per-person contact rates for each individual in population age group $b$, $\alpha$ is a baseline parameter,
$\bm{x}_i$ are $P$-dimensional socio-demographic variables of participant $i$ that multiplicatively mediate contact intensity surfaces through the $P$ fixed-effects coefficients $\beta = (\beta_1, \beta_2, \ldots, \beta_p)^\top \in\mathbb{R}^P$. Expanding Eq.~\ref{e:flow_identity} to $P_a P_b \gamma_{a,b} = P_b P_a \gamma_{b,a}$, it is clear that the 2D random function $\pmb{f}$ is symmetric in $a$ and $b$, i.~e. $\pmb{f}(a,b) = \pmb{f}(b,a)$ for all $a, b \in\mathcal{A}$. This symmetry explains how the BRC leverages information to decipher fine-age contact intensity surfaces from coarse data, and also clarifies that computational gains can be made by concentrating on upper triagonal matrices. Reporting fatigue effects are adjusted for through the non-negative function $\rho_{\bm{x}_i}(r_i)$, which is parameterised in terms of the number of repeat participations $r_i$ of individual $i$ and may additionally differ by socio-demographic attributes $\bm{x}_i$ of individual $i$. 

==> supp_methods_old.tex <==
\subsection*{Identifying individual-level factors associated with the number of daily social contacts and reporting fatigue.}
%
We here describe our approach to identifying factors associated with the number of daily social contacts and reporting fatigue associated with repeat survey participation. Let $Y^0_i$ for $i = 1,2,\ldots, n_0$ and $Y^1_i$ for $i = 1,2,\ldots, n_1$ denote the number of contacts by a first-time participant and a repeating participant, respectively. We implemented a two-stage variable selection process where the variables relevant to the number of daily social contacts are selected in the first stage using data from first-time participants, and those variables further associated with reporting fatigue are identified in the second stage. The COVIMOD survey included two waves with a good balance of first-time participants and repeating participants, waves 4 and waves 21. We identified variables associated with the number of daily social contacts and reporting fatigue first on wave 4, and then tested if the same variables were also identified in wave 21 to assess the robustness in variable selection procedures. The final selected variables were the union of the selected variables from both waves. A complete list of candidate variables and selection results can be found in Table~\ref{tab:varselect-variables}. 

In the first stage, we analysed data from first-time participants and considered the model
\begin{subequations}\label{eq:stage-1-varselect}
\begin{align}
    Y^0_i &\sim \text{Poisson}(\lambda_i) \quad \text{for } i = 1,2,\ldots,n_0 \\
    \log(\lambda_i) &= \beta_0 + \bm{u}^\top_i \alpha + \bm{v}^\top_i \beta
\end{align}
\end{subequations}
where $\bm{u}_i$ is a vector consisting of covariates that are well-established for their association with heterogeneity in count intensities (gender, age, household size)~\cite{wong_social_2023, dan_estimating_2023, backer_contact_2024,  gimma_changes_2022, tomori_individual_2021, loedy_longitudinal_2023}, and $\bm{v}_i$ is a vector of further putative covariates that could be associated with heterogeneity in count intensities, which we tested through regularised horseshoe (RHS) variable selection~\cite{piironen_sparsity_2017}. We assigned generic un-informative priors to $\beta_0$ and $\alpha = (\alpha_1, \alpha_2, \ldots, \alpha_J)^\top$, 
\begin{align*}
    \beta_0 &\sim \text{Normal}(0, 100) \\
    \alpha_j &\sim \text{Normal}(0, \sigma^2_\alpha) \quad j = 1,2,\ldots,J \\
    \sigma_\alpha &\sim \text{half-Cauchy}^+(0, 1),
\end{align*}
and RHS priors to $\beta = (\beta_1, \beta_2, \ldots, \beta_K)^\top$,
\begin{subequations}\label{eq:horseshoe-prior}
\begin{align}
\beta_k | \zeta_k, \varepsilon, c &\sim \text{Normal}(0, \varepsilon^2\tilde{\zeta}_k^2), \quad \tilde{\zeta}_k^2 = \frac{c^2\zeta_k^2}{c^2 + \varepsilon^2\zeta^2_k}\label{eq:horseshoe-prior-a} \\
\zeta_k &\sim \text{student-}t^+_{\nu_1}(0,1), \quad k = 1,\ldots,K \\
c^2 &\sim \text{Gamma}(\nu_2, \nu_2 s^2/2) \\
\varepsilon &\sim \text{student-}t^+_{\nu_3}(0, \varepsilon_0),
\end{align}
\end{subequations}
where the scaling parameter $\varepsilon_0$ for $\varepsilon$ was expressed as 
\begin{equation*}
    \varepsilon_0 = \frac{p_0}{P-p_0} \frac{1}{n},
\end{equation*}
with $P$ the number of covariates in the model and $p_0 \in \{0, \dotsc, K\}$ specified to reflect prior knowledge on the effective number of non-zero coefficients~\cite{piironen_sparsity_2017}. For succinctness, we denote this prior as
\begin{equation*}
    \beta_k \sim \text{RHS}_{\nu_1,\nu_2,\nu_3}(s^2, p_0).
\end{equation*}
We set the hyperparameters of the RHS prior to $\nu_1 = 3, \nu_2 = 2, \nu_3 = 4, s^2 = 2$ to facilitate sampling in {\it Stan}~\cite{piironen_sparsity_2017}, and $p_0 = K/2$ to obtain a weakly informative prior on the number of selected variables. Following inference, variables were retained if the absolute medium effect size of their corresponding coefficient was less than or greater than $\log(1.05) \approx 0.049$, which corresponds to a 5\% change from the population average contact rate $\exp(\beta_0)$. We performed a sensitivity analysis where $p0$ was set to 1 (strong shrinkage) or $K - 1$ (weak shrinkage). Both settings did not change the features that were selected.

In the second stage, we retained the selected coefficients and investigated the presence of reporting fatigue on the data from repeating participants through the model
\begin{subequations}\label{eq:stage-2-varselect}
\begin{align}
    Y^1_i &\sim \text{Poisson}(\lambda_i) \quad \text{for } i = 1,2,\ldots,n_1 \\
    \log(\lambda_i) &= \hat\beta_0 + \bm{u}^\top_i \hat{\alpha} + \bm{v}^\top_i \hat{\beta}+ \bm{w}^\top_i \gamma, 
\end{align}
\end{subequations}
where $\hat\beta_0$, $\hat{\alpha}$, and $\hat{\beta}$ denote the posterior median point estimates from model~\eqref{eq:stage-1-varselect} fitted to data from first-time participants (without using the RHS prior), and $\bm{w}_i$ is a vector consisting of covariates putatively associated with reporting fatigue. As fatigue should only have negative effects on contact intensity, we constrained $\bm{\gamma}$ to only take negative values. This was done by replacing  Eq.~\eqref{eq:horseshoe-prior-a} with a half-normal prior such that $\gamma_l | \zeta_l, \varepsilon, c \sim \text{half-Normal}^{-}(0, (1-2/\pi)^{-1} \varepsilon^2 \tilde{\zeta}^2_l)$ for $l = 1,2,\ldots,L$. For simplicity, we denote the constrained RHS prior as
\begin{equation}
    \gamma_l \sim \text{half-RHS}^{-}_{\nu_1,\nu_2,\nu_3}(s^2, p_0).
\end{equation}
The adjustment factor $(1-2/\pi)^{-1}$ in the scale component of the half normal was added to ensure that the prior variance of the constrained RHS prior is equivalent to that of the non-constrained version. As in the first-stage analysis, we set the hyperparameters of the RHS prior to $\nu_1 = 3, \nu_2 = 2, \nu_3 = 4, s^2 = 2$~\cite{piironen_sparsity_2017}, and $p_0 = L/2$. All inference in this work was performed using the \textit{Stan}\cite{stan_development_team_stan_2022} probabilistic programming language through the \textit{cmdstanr}\cite{jonah_gabry_cmdstanr_2023} package version 2.34.1 as front-end. 

\subsection*{Investigating the functional form of reporting fatigue effects over the number of repeat participations}
Here, we describe our approach to identifying the functional form of reporting fatigue with the number of times individuals participate in the study. Let $Y_{i,r}$ denote the number of contacts reported by individual $i$ in their $r$-th participation, with $i=1,\dotsc,N$ and $r=0,1,\dotsc,R$. Additionally, we introduce the index map $t_{i,r}$ that identifies the wave that individual $i$ had at their $r$-th participation. For instance, if the third repeat ($r = 3$) of the first participant ($i=1$) was reported during the $4$-th wave, then $t_{i,r} =  4$. $Y_{i,0}$ corresponds to the number of contacts reported the first-time that individual $i$ participated in the study. Further, let $\bm{x}_{i,r} = (x_{i,1}, \ldots, x_{i,J})^\top$ denote a $J$ dimensional vector containing the covariates selected in the previous variable selection analysis along with age, gender, and household size.

We assessed increasingly less complex Bayesian Negative Binomial count models in their ability to describe mean trends in $Y_{i,r}$, and all these models had the following common components, 
\begin{subequations}\label{eq:longitudinal-model}
\begin{align}
 Y_{i,r} &\sim \text{NegBinomial}(\lambda_{i,r}, \varphi) \\
\log(\lambda_{i,r}) &= \beta_0 + \bm{x}_{i,r}^\top\beta + \tau(t_{i,r}) + \rho(r) \\
\tau(t) &\sim \text{GP}(0, k),   
\end{align}
\end{subequations}
where $\varphi$ denotes a real-valued overdispersion parameter such that the mean and variance of the Negative Binomial observation model are $\E{Y_{i,r}} = \lambda_{i,r}$ and $\Var{Y_{i,r}} = \lambda_{i,r} + \lambda_{i,r}^2/\varphi$. The latent random variable $\alpha$ is the baseline term, and $\beta = (\beta_1, \ldots, \beta_J)^\top$ is a vector of coefficients for the individuals' characteristics, and calendar-time effects are modelled as deviations from the baseline $\alpha$ through a zero-mean Gaussian process characterised by the Mat\'ern 3/2 covariance kernel
\begin{equation}
k(t, t')  = \sigma_{\tau} \left(1 + \frac{\sqrt{3}|t - t'|}{\ell_\tau} \right) \exp\left( -\frac{\sqrt{3}|t - t'|}{\ell_\tau} \right).  
\end{equation}
Throughout, we used the following generic priors to the parameters in the components common across all models:
\begin{subequations}
\begin{align}
1/\varphi &\sim \text{Exponential}(1), \\
\beta_0 &\sim \text{Normal}(0, 10), \\
\beta_j &\overset{i.i.d}{\sim} \text{Normal}(0, \sigma^2_{\beta}) \quad j = 1,\ldots,J \\
\sigma_{\beta} &\sim \text{Cauchy}^+(0,1) \\
\sigma_{\tau}, \ell_{\tau} &\overset{i.i.d.}{\sim} \text{inv-Gamma}(5, 1).
\end{align}
\end{subequations}
We considered three different approaches for capturing the functional form on how  reporting fatigue accumulates with the number of repeat participation. The first model comprised $R$ independent reporting fatigue effects 
\begin{equation}
    \rho_r \overset{i.i.d.}{\sim} \text{Normal}(0, 1) \quad r \in \{1,2,\ldots,R\},
\end{equation}
with $\rho_{r=0}$ set to $0$ for identifiability. This first model imposes no specific functional form of reporting fatigue with $r$. The second model was a non-parametric Gaussian process prior with squared exponential kernel depending on rescaled repeat times $\tilde{r} = (r - \text{mean})/\text{sd-dev}$
\begin{subequations}
\begin{align}
    \rho^{\text{GP}}(\tilde{r}) & \sim \text{GP}(0, k_{\text{SE}})\\
    k_{\text{SE}}(\tilde{r},\tilde{r}') & = \sigma_\rho \exp\left( -\frac{(\tilde{r}-\tilde{r}')^2}{2 \ell_\rho^2} \right) \\
    \sigma_{\rho}, \ell_{\rho} &\overset{i.i.d.}{\sim} \text{inv-Gamma}(5, 1)
\end{align}
\end{subequations}
for $r=1,\dotsc,R$, and $\rho^{\text{GP}}=0$ for $r=0$ to ensure identifiability. This model imposes smooth trends on reporting fatigue effects with the number of repeat participations, and consequently renders reporting fatigue effects more predictable.
\begin{figure}
    \centering
    \includegraphics{figures/hill_function.pdf}
    \caption{Functional form of the Hill function under different parameter values.}
    \label{fig:hill-function}
\end{figure}
For the third model, we take inspiration from dose-response modeling in biochemistry~\cite{prinz_hill_2009} and model reporting fatigue with a three-parameter Hill function:
\begin{equation}\label{eq:hill-function}
    \rho^{\text{Hill}}(r) = -\gamma \frac{e^\zeta r^\eta}{1 + e^\zeta r^\eta} \quad \text{where} \quad \gamma, \eta \in \mathbb{R}^+, \zeta \in \mathbb{R}
\end{equation}
where $\gamma$ is a scale parameter which control the effect size at large values of $r$, while $\zeta$ and $\eta$ in tandem controls how quickly the function approaches its minimum value. Figure~\ref{fig:hill-function} shows the functional form of the Hill function under different parameter values. This model is computationally more efficient than GP models, and renders due to its parametric form reporting fatigue effects strongly predictable. Given their constraints, we assign the following priors to each parameter:
\begin{align*}
    \gamma &\sim \text{half-Normal}^+(0,1) \\
    \zeta &\sim \text{Normal}(0,1) \\
    \eta &\sim \text{Exponential}(1).
\end{align*}

\subsection*{Generalised additive model for fine-age contact intensity with reporting fatigue adjustment}
 %Now, we merge the insights from the two previous models to estimate marginal social contact intensities from data potentially corrupted by reporting fatigue. We selected data from COVIMOD wave 21, which includes a mix of first-time and multiple-time participants, and was collected after the second wave of COVID-19 lockdowns in Germany, minimizing the impact of contact reduction measures on our analysis.

%Our objectives are twofold: the first is to validate a method for correcting the effects of reporting fatigue in existing datasets, and second is to determine the threshold of participant repeats beyond which fatigue significantly skews the data, despite statistical corrections. We begin by splitting the data based on the participants' number of repeats. We fit a model on a subset of the data with only first-time participants, and treat the estimates we obtain as the reference or \textit{pseudo-truth}. We then add back the splits containing participants with repeats in an incremental fashion, assessing at each step the mean square error (MSE) and the proportion of estimates within the 95\% confidence interval (CI) relative to the psuedo-truth. This approach helps us evaluate how well our adjustment works and identify the maximum number of repeat participation we can include before data reliability declines. The following text details the construction of our proposed model.

Let $a_i$ denote the age of participant, $\bm{u}_i = (u_{i1}, \ldots, u_{iP})^\top \in \{0,1\}^P$ denote the vector of gender and household size variables, and $\bm{w}_i = (w_{i1}, \ldots, w_{iQ})^\top \in \{0,1\}^Q$ denote the vector of covariates associated with reporting fatigue identified in the variable selection analysis. We consider the following negative binomial generalised additive count model,
\begin{subequations} \label{eq:gam}
\begin{align}
    Y_{i,r} &\sim \text{NegBinomial}\left( \lambda_{i,r}, \varphi \right), \\
    \log(\lambda_{i,r}) &= \beta_0 + \bm{u}_i^\top \beta + f_\theta(a_i) + \bm{w}^\top_i \rho(r)
\end{align}
\end{subequations}
where $\beta_0$ is a global baseline parameter and $\rho(r) \in \mathbb{R}^Q$ is a vector consisting of elements
\begin{align*}
    [\rho(r)]_q = -\gamma_q \exp(\zeta_q)r^{\eta_q}/(1+\exp(\zeta_q)r^{\eta_q})
\end{align*}
which models the fatigue effect at each repeat for the selected variables.
$\alpha$ and the covariate parameter vector $\beta = (\beta_1, \beta_2, \ldots, \beta_p)^\top$ are assigned generic Gaussian priors, and the reciprocal of the overdispersion parameter $\varphi$ is given an exponential prior:
\begin{align*}
    \beta_0 &\sim \text{Normal}(0, 10), \\
    \beta_p &\overset{i.i.d.}{\sim} \text{Normal}(0, 1), \quad p = 1,\ldots,P \\
    1/\varphi &\sim \text{Exp}(1).
\end{align*}
Let $\hat\gamma, \hat\zeta$, and $\hat\eta$ denote the posterior median estimates from Eq.~\ref{eq:longitudinal-model}. Leveraging the Bayesian framework to reflect prior knowledge, we assign the following informative priors to the parameters of the hill function,
\begin{align*}
    \gamma_q &\overset{i.i.d.}{\sim} \text{half-Normal}^+(\hat\gamma, 0.5), \\
    \zeta_q &\overset{i.i.d.}{\sim} \text{Normal}(\hat\zeta, 0.1), \\
    \eta_q &\overset{i.i.d.}{\sim} \text{half-Normal}^+(\hat\eta, 0.1).
\end{align*}
$f_\theta(a_i): \mathbb{R} \mapsto \mathbb{R}$ is a non-linear function that describes the effect of participant age on the rate of contact. For computational efficiency, $f_\theta$ is modeled using the zero-mean Hilbert space approximate Gaussian process~\cite{solin_hilbert_2020, riutort-mayol_practical_2022} (HSGP) which is parametrised by $\theta = (\sigma, \ell)$ and characterised by the squared exponential covariance kernel:
\begin{equation*}
    k(x, x') = \sigma \exp\left( -\frac{(x - x')^2}{2\ell^2} \right).
\end{equation*}

\subsection*{Fatigue adjusted estimates for all waves of COVIMOD}
To obtain fatigue adjusted estimates for all 33 waves of the COVIMOD surveys, we applied the GAM described in the previous section (Eq.~\ref{eq:gam}) in the following manner. Let $t = 1,2,\ldots,33$ be an index for the waves. For the first wave ($t = 1$), priors were unchanged from those defined in the previous section. From the second wave onwards, priors for the parameters of the individual covariates and hill functions were set as,
\begin{align*}
    \beta_{t,p} \sim \text{Normal}(\hat\beta_{t-1,p}, 0.3) \quad \text{for } p = 1,2,\ldots,P
\end{align*}
and
\begin{align*}
    \gamma_{t,q} &\sim \text{half-Normal}^+(\hat\gamma_{t-1,q}, 0.3) \\
    \zeta_{t,q} &\sim \text{Normal}(\hat\zeta_{t-1,q}, 0.1) \\
    \eta_{t,q} &\sim \text{half-Normal}^+(\hat\eta_{t-1,q}, 0.1) \quad \text{for } q = 1,2,\ldots,Q.
\end{align*}
Here, $\hat\beta_{t-1,p}, \hat\gamma_{t-1,q}, \hat\zeta_{t-1,q}$, and $\hat\eta_{t-1,q}$ denote the posterior mean of the parameters from the previous wave. This sequential fitting process allows the model to partially leverage information from previous waves to resolve an un-identifiability issue between $\beta_{t,p}$ and the parameters of the Hill function when there are no first-time participants in the data. For the model based fatigue unadjusted estimates, this identifiability issue did not exist and hence estimates were obtained by fitting the model independently to data from each wave. 

==> tables/varselect_baseline.tex <==
\begin{table}[h]
\caption{Summary Statistics of baseline parameters from the variable selection model}
\centering
\begin{tabular}[t]{rcccccc}
\toprule
Characteristic & Posterior median & 2.5\% quantile & 97.5\% quantile & $\hat{R}$ & ESS bulk & ESS tail\\
\midrule
Nursery/Pre-shool [0-5] & 0.41 & 0.25 & 0.86 & 1.01 & 1389.83 & 1128.73\\
Raised-at-home-toddler [0-5] & 0.19 & 0.04 & 0.64 & 1.01 & 1389.61 & 1130.58\\
Student [6-9] & 0.11 & -0.04 & 0.56 & 1.01 & 1391.41 & 1131.38\\
Student [10-14] & 0.21 & 0.05 & 0.66 & 1.01 & 1389.30 & 1127.54\\
\addlinespace
15-19 & 0.45 & 0.33 & 0.54 & 1.00 & 3004.88 & 3643.21\\
20-24 & 0.01 & -0.11 & 0.09 & 1.00 & 3001.70 & 3647.94\\
25-34 & 0.00 & -0.11 & 0.09 & 1.00 & 3001.25 & 3613.40\\
35-44 & -0.20 & -0.31 & -0.11 & 1.00 & 2999.47 & 3598.38\\
45-54 & 0.11 & 0.00 & 0.20 & 1.00 & 2995.16 & 3623.93\\
55-64 & -0.06 & -0.18 & 0.03 & 1.00 & 2980.26 & 3566.13\\
65-69 & -0.02 & -0.13 & 0.07 & 1.00 & 2949.93 & 3632.71\\
70-74 & -0.14 & -0.26 & -0.05 & 1.00 & 2988.46 & 3646.69\\
75-79 & -0.17 & -0.28 & -0.08 & 1.00 & 2989.16 & 3613.80\\
80-84 & -0.34 & -0.46 & -0.25 & 1.00 & 3194.60 & 3613.68\\
\addlinespace
Male & 0.00 & -0.18 & 0.17 & 1.00 & 3703.47 & 4643.30\\
Female & 0.00 & -0.18 & 0.17 & 1.00 & 3693.84 & 4621.94\\
\addlinespace
1 person household & 0.06 & -0.04 & 0.14 & 1.00 & 6239.02 & 10733.11\\
2 person household & -0.03 & -0.13 & 0.05 & 1.00 & 6251.21 & 10747.82\\
3 person household & -0.03 & -0.12 & 0.05 & 1.00 & 6238.17 & 10470.88\\
4 person household & 0.03 & -0.06 & 0.11 & 1.00 & 6239.24 & 10489.81\\
\addlinespace
Employed [full-time] & 0.02 & -0.10 & 0.47 & 1.01 & 1543.86 & 1032.26\\
Employed [part-time] & 0.05 & -0.08 & 0.49 & 1.01 & 1543.95 & 1050.97\\
Full-time parent, homemaker & -0.64 & -0.77 & -0.20 & 1.01 & 1546.08 & 1086.43\\
Long-term sick or disabled & -0.54 & -0.66 & -0.09 & 1.01 & 1547.11 & 1032.39\\
Retired & -0.46 & -0.59 & -0.01 & 1.01 & 1544.85 & 1039.70\\
Self employed & -0.09 & -0.22 & 0.35 & 1.01 & 1544.06 & 1077.03\\
Student/Pupil & -0.28 & -0.40 & 0.17 & 1.01 & 1542.97 & 1018.11\\
Unemployed [not seeking job] & -0.71 & -0.83 & -0.26 & 1.01 & 1545.83 & 1014.50\\
Unemployed [seeking job] & -0.48 & -0.61 & -0.03 & 1.01 & 1544.54 & 1034.63\\
\bottomrule
\end{tabular}
\end{table}

==> tables/varselect_repeat.tex <==
\begin{table}[h]
\caption{Percent decrease in the average number of reported contacts after repeat associated with each individual characteristic}
\centering
\begin{tabular}[t]{rcccccc}
\toprule
Characteristic & Posterior median & 2.5\% quantile & 97.5\% quantile & Rhat & ESS bulk & ESS tail\\
\midrule
Nursery/Pre-shool [0-5] & -70.77 & -71.27 & -70.28 & 1 & 15475.73 & 14552.48\\
Raised-at-home-toddler [0-5] & -65.34 & -66.49 & -64.11 & 1 & 15221.10 & 12317.15\\
Student [6-9] & -47.26 & -48.08 & -46.43 & 1 & 15418.65 & 13255.89\\
Student [10-14] & -53.59 & -54.04 & -53.14 & 1 & 15719.36 & 14964.55\\
15-19 & 0.00 & -0.01 & 0.00 & 1 & 10502.40 & 8032.19\\
\addlinespace
20-24 & -14.60 & -15.76 & -13.43 & 1 & 16168.32 & 10835.91\\
25-34 & 0.00 & -0.02 & 0.00 & 1 & 3594.55 & 2000.26\\
35-44 & 0.00 & -0.03 & 0.00 & 1 & 10930.45 & 6941.73\\
45-54 & -32.60 & -33.01 & -32.19 & 1 & 15667.09 & 14980.83\\
55-64 & -1.15 & -1.68 & -0.60 & 1 & 12662.89 & 8911.66\\
\addlinespace
65-69 & -1.58 & -2.13 & -1.02 & 1 & 14266.88 & 10181.73\\
70-74 & -0.02 & -0.10 & 0.00 & 1 & 9773.80 & 6940.91\\
75-79 & -9.78 & -10.91 & -8.60 & 1 & 15295.21 & 10611.75\\
80-84 & -0.05 & -0.27 & 0.00 & 1 & 9980.15 & 6857.86\\
Male & 0.00 & -0.01 & 0.00 & 1 & 11238.31 & 7997.14\\
\addlinespace
Female & 0.00 & -0.01 & 0.00 & 1 & 11238.28 & 6720.93\\
1 person household & -8.12 & -8.61 & -7.62 & 1 & 15506.31 & 14854.17\\
2 person household & -16.78 & -17.24 & -16.31 & 1 & 15135.76 & 14426.45\\
3 person household & -11.12 & -11.56 & -10.66 & 1 & 14578.67 & 14974.50\\
4 person household & 0.00 & -0.01 & 0.00 & 1 & 10940.86 & 7354.91\\
\addlinespace
Employed [full-time] & -12.82 & -13.21 & -12.42 & 1 & 16179.78 & 15094.43\\
Employed [part-time] & -9.43 & -9.96 & -8.90 & 1 & 15209.95 & 14534.20\\
Full-time parent, homemaker & -0.01 & -0.03 & 0.00 & 1 & 8752.63 & 5518.47\\
Long-term sick or disabled & -0.02 & -0.12 & 0.00 & 1 & 12200.31 & 8870.22\\
Retired & 0.00 & -0.01 & 0.00 & 1 & 9531.29 & 7194.26\\
\addlinespace
Self employed & -32.72 & -33.33 & -32.10 & 1 & 15898.10 & 15222.41\\
Student/Pupil & -27.69 & -28.25 & -27.13 & 1 & 15853.51 & 15155.13\\
Unemployed [not seeking job] & -31.15 & -32.69 & -29.59 & 1 & 15633.53 & 12148.04\\
Unemployed [seeking job] & -0.01 & -0.05 & 0.00 & 1 & 5921.37 & 3796.69\\
\bottomrule
\end{tabular}
\end{table}
